Characterizations of Morse quasi-geodesics via superlinear divergence and sublinear contraction

We introduce and begin a systematic study of sublinearly contracting projections. We give two characterizations of Morse quasi-geodesics in an arbitrary geodesic metric space. One is that they are sublinearly contracting; the other is that they have completely superlinear divergence. We give a further characterization of sublinearly contracting projections in terms of projections of geodesic segments.

==> abstract.tex <==
%!TEX root = Main.tex
We introduce and begin a systematic study of sublinearly contracting
projections.

We give two characterizations of Morse quasi-geodesics in an arbitrary geodesic
metric space. One is that they are sublinearly contracting; the other
is that they have completely superlinear divergence.

We give a further characterization of sublinearly contracting projections in terms
of projections of geodesic segments.
\endinput

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "Main"
%%% End: 


==> contraction.tex <==






\endinput
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

